Quasimorphisms on the group of density preserving diffeomorphisms of the M\"{o}bius band

The existence of quasimorphisms on groups of homeomorphisms of manifolds has been extensively studied under various regularity conditions, such as smooth, volume-preserving, and symplectic. However, in this context, nothing is known about groups of `area'-preserving diffeomorphisms on non-orientable manifolds. In this paper, we initiate the study of groups of density-preserving diffeomorphisms on non-orientable manifolds. Here, the density is a natural concept that generalizes volume without concerning orientability. We show that the group of density-preserving diffeomorphisms on the M\"obius band admits countably many unbounded quasimorphisms which are linearly independent. Along the proof, we show that groups of density preserving diffeomorphisms on compact, connected, non-orientable surfaces with non-empty boundary are weakly contractible.

==> header_labeling.tex <==
\makeatletter
\let\c@equation\c@subsection
\makeatother
\numberwithin{equation}{section} 

\makeatletter
\let\c@figure\c@equation
\makeatother
\numberwithin{figure}{section} 


\theoremstyle{plain}
\newtheorem{thm}[equation]{Theorem}
\newtheorem{cor}[equation]{Corollary}
\newtheorem{lem}[equation]{Lemma}
\newtheorem{conj}[equation]{Conjecture}
\newtheorem{prop}[equation]{Proposition}


%%%https://tex.stackexchange.com/questions/291346/marking-the-end-of-a-definition
%%%see egreg's solution.
\theoremstyle{definition}
\newtheorem{defn/}[equation]{Definition}
\newtheorem{ex}[equation]{Example}
\newtheorem{fact}[equation]{Fact}
\newtheorem{ques}[equation]{Question}
\newtheorem{const/}[equation]{Construction}
\newtheorem{conv/}[equation]{Convention}

%%%https://tex.stackexchange.com/questions/126711/double-slash-close-together
\newcommand{\sslash}{\mathbin{\medslash\mkern-7mu\medslash}}

\newenvironment{defn}
  {\renewcommand\qedsymbol{$\sslash$} 
  \pushQED{\qed} \begin{defn/}}
  {\popQED \end{defn/}}
\newenvironment{const}
  {\renewcommand\qedsymbol{$\sslash$} 
  \pushQED{\qed} \begin{const/}}
  {\popQED \end{const/}}
\newenvironment{conv}
  {\renewcommand\qedsymbol{$\sslash$} 
  \pushQED{\qed} \begin{conv/}}
  {\popQED \end{conv/}}
  

\theoremstyle{remark}
\newtheorem{rmk/}[equation]{Remark}
\newtheorem*{rmk*}{Remark}
\newtheorem{case}{Case}
\newtheorem*{case*}{Case}
\renewcommand{\thecase}{\Roman{case}}
\newtheorem{claim}[equation]{Claim}
\newtheorem*{claim*}{Claim}



\newenvironment{rmk}
  {\renewcommand{\qedsymbol}{$\sslash$}
   \pushQED{\qed}\begin{rmk/}}
  {\popQED\end{rmk/}}




\newcommand{\refsec}[1]{Section~\ref{Sec:#1}}
\newcommand{\refapp}[1]{Appendix~\ref{App:#1}}
\newcommand{\refthm}[1]{Theorem~\ref{Thm:#1}}
\newcommand{\refcor}[1]{Corollary~\ref{Cor:#1}}
\newcommand{\reflem}[1]{Lemma~\ref{Lem:#1}}
\newcommand{\refprop}[1]{Proposition~\ref{Prop:#1}}
\newcommand{\refclm}[1]{Claim~\ref{Clm:#1}}
\newcommand{\refrmk}[1]{Remark~\ref{Rmk:#1}}
\newcommand{\refexa}[1]{Example~\ref{Exa:#1}}
\newcommand{\refconv}[1]{Convention~\ref{Conv:#1}}
\newcommand{\refconst}[1]{Construction~\ref{Const:#1}}
\newcommand{\reffac}[1]{Fact~\ref{Fac:#1}}
\newcommand{\refque}[1]{Question~\ref{Que:#1}}
\newcommand{\reffig}[1]{Figure~\ref{Fig:#1}}
\newcommand{\reftab}[1]{Table~\ref{Tab:#1}}
\newcommand{\refdefn}[1]{Definition~\ref{Defn:#1}}
\newcommand{\refeqn}[1]{Equation~\ref{Eqn:#1}}
\newcommand{\refconj}[1]{Conjecture~\ref{Conj:#1}}
\newcommand{\refitm}[1]{(\ref{Itm:#1})}



\newcommand{\fakeenv}{} %%% prints the emptystring

%%% For theorem style
\newenvironment{restate}[2]  %%% restate takes two arguments 
{ 
 \renewcommand{\fakeenv}{#2} %%% So now \fakeenv prints #2
 \theoremstyle{plain} 
 \newtheorem*{\fakeenv}{#1~\ref{#2}} %%% so now #2 is the name of a
 %%% theorem-like environment.   
 \begin{\fakeenv}
}
{
 \end{\fakeenv}
}

